Not the Silver Bullet: LLM-enhanced Programming Error Messages are Ineffective in Practice

The sudden emergence of large language models (LLMs) such as ChatGPT has had a disruptive impact throughout the computing education community. LLMs have been shown to excel at producing correct code to CS1 and CS2 problems, and can even act as friendly assistants to students learning how to code. Recent work shows that LLMs demonstrate unequivocally superior results in being able to explain and resolve compiler error messages -- for decades, one of the most frustrating parts of learning how to code. However, LLM-generated error message explanations have only been assessed by expert programmers in artificial conditions. This work sought to understand how novice programmers resolve programming error messages (PEMs) in a more realistic scenario. We ran a within-subjects study with $n$ = 106 participants in which students were tasked to fix six buggy C programs. For each program, participants were randomly assigned to fix the problem using either a stock compiler error message, an expert-handwritten error message, or an error message explanation generated by GPT-4. Despite promising evidence on synthetic benchmarks, we found that GPT-4 generated error messages outperformed conventional compiler error messages in only 1 of the 6 tasks, measured by students' time-to-fix each problem. Handwritten explanations still outperform LLM and conventional error messages, both on objective and subjective measures.

==> tables/participant-experience-c-only.tex <==
\begin{tabular}{@{}lrl@{}}
  \toprule
  Experience & \(n\) & \\
  \midrule
  None                       & 8  & \inlinebar{0.56}  \\
  Very little (0--3 months)  & 32 & \inlinebar{2.25}  \\
  Some (3--6 months)         & 26 & \inlinebar{1.83}  \\
  A good deal (6--12 months) & 16 & \inlinebar{1.12}  \\
  A lot (1--2 years)         & 13 & \inlinebar{0.91}  \\
  Extensive (2+ years)       & 11 & \inlinebar{0.77}  \\
  \bottomrule
\end{tabular}


==> tables/participant-experience.tex <==
% Assuming:
% booktabs is loaded
% the \inlinebar{} command is defined
\begin{tabular}{@{}llrl@{}}
  \toprule
  Language & Experience                 & \(n\) & \\
  \midrule
  C        & None                       & 8     & \inlinebar{0.56}  \\
           & Very little (0--3 months)  & 32    & \inlinebar{2.25}  \\
           & Some (3--6 months)         & 26    & \inlinebar{1.83}  \\
           & A good deal (6--12 months) & 16    & \inlinebar{1.12}  \\
           & A lot (1--2 years)         & 13    & \inlinebar{0.91}  \\
           & Extensive (2+ years)       & 11    & \inlinebar{0.77}  \\
  \midrule
  Python   & None                       & 2     & \inlinebar{0.14}  \\
           & Very little (0--3 months)  & 11    & \inlinebar{0.77}  \\
           & Some (3--6 months)         & 4     & \inlinebar{0.28}  \\
           & A good deal (6--12 months) & 3     & \inlinebar{0.21}  \\
           & A lot (1--2 years)         & 1     & \inlinebar{0.07}  \\
           & Extensive (2+ years)       & 2     & \inlinebar{0.14}  \\
  \bottomrule
\end{tabular}


==> tables/per-tasks-compairison-beta.tex <==
\begin{tabular}{@{}lrlrlr@{}}
\toprule
Task                        & \multicolumn{5}{l}{Comparisons}                                \\ \midrule
Flipped assignment          & Handwritten & =              & GCC    & =             & GPT-4  \\
                            & 33.2s       &                & 36.8s  &               & 49.5s  \\
\#const instead of \#define & Handwritten & \textless{}**  & GPT-4  & =             & GCC    \\
                            & 32.1s       &                & 71.2s  &               & 76.0s  \\
Using a keyword as a name   & Handwritten & \textless{}*** & GPT-4  & \textless{}** & GCC    \\
                            & 38.3s       &                & 73.1s  &               & 101.7s \\
Missing parameter           & Handwritten & =              & GCC    & \textless{}*  & GPT-4  \\
                            & 45.2s       &                & 45.8s  &               & 60.9s  \\
Missing curly brace         & Handwritten & \textless{}*** & GPT-4  & =             & GCC    \\
                            & 30.7s       &                & 102.4s &               & 153.0s \\
Reassigning a constant      & Handwritten & \textless{}*   & GPT-4  & =             & GCC    \\
                            & 65.6s       &                & 117.3s &               & 123.6s \\ \bottomrule
\end{tabular}

==> tables/regression.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Wed, Apr 10, 2024 - 15:22:53
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\toprule \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cmidrule{2-2} 
\\[-1.8ex] & log(time\_to\_complete) \\ 
\midrule \\[-1.8ex] 
 taskinvalid-define & 0.515$^{***}$ (0.146) \\ 
  taskkeyword-as-identifier & 0.883$^{***}$ (0.159) \\ 
  taskmissing-param & 0.082 (0.145) \\ 
  taskmissing-semicolon & 1.057$^{***}$ (0.149) \\ 
  taskmodifying-const & 0.948$^{***}$ (0.156) \\ 
  conditionHandwritten & $-$0.150 (0.152) \\ 
  conditionGPT-4 & 0.084 (0.145) \\ 
  exercise\_id & $-$0.116$^{***}$ (0.014) \\ 
  taskinvalid-define:conditionHandwritten & $-$0.467$^{**}$ (0.207) \\ 
  taskkeyword-as-identifier:conditionHandwritten & $-$0.841$^{***}$ (0.221) \\ 
  taskmissing-param:conditionHandwritten & 0.252 (0.209) \\ 
  taskmissing-semicolon:conditionHandwritten & $-$1.255$^{***}$ (0.210) \\ 
  taskmodifying-const:conditionHandwritten & $-$0.363$^{*}$ (0.211) \\ 
  taskinvalid-define:conditionGPT-4 & $-$0.044 (0.209) \\ 
  taskkeyword-as-identifier:conditionGPT-4 & $-$0.461$^{**}$ (0.208) \\ 
  taskmissing-param:conditionGPT-4 & 0.232 (0.205) \\ 
  taskmissing-semicolon:conditionGPT-4 & $-$0.314 (0.209) \\ 
  taskmodifying-const:conditionGPT-4 & $-$0.064 (0.211) \\ 
  Constant & 4.160$^{***}$ (0.117) \\
\midrule \\[-1.8ex] 
Observations & 623 \\ 
Log Likelihood & $-$567.427 \\ 
Akaike Inf. Crit. & 1,172.854 \\ 
\bottomrule \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 


==> tables/skips.tex <==
\begin{tabular}{lrrr}
  \toprule
  \multirow{2}{*}{Task}       & \multicolumn{3}{c}{Condition} \\ \cmidrule{2-4}
                              & GCC  & Handwritten & GPT-4 \\
  \midrule
  Flipped assignment          & 0    & 0           & 1 \\
  \#const instead of \#define & 2    & 0           & 0 \\
  Using a keyword as a name   & 4    & 0           & 0 \\
  Missing parameter           & 1    & 0           & 0 \\
  Missing curly brace         & 3    & 0           & 2 \\
  Reassigning a constant      & 0    & 0           & 0 \\
  \bottomrule
\end{tabular}

